Incremental Calibration of Architectural Performance Models with Parametric Dependencies

Architecture-based Performance Prediction (AbPP) allows evaluation of the performance of systems and to answer what-if questions without measurements for all alternatives. A difficulty when creating models is that Performance Model Parameters (PMPs, such as resource demands, loop iteration numbers and branch probabilities) depend on various influencing factors like input data, used hardware and the applied workload. To enable a broad range of what-if questions, Performance Models (PMs) need to have predictive power beyond what has been measured to calibrate the models. Thus, PMPs need to be parametrized over the influencing factors that may vary. Existing approaches allow for the estimation of parametrized PMPs by measuring the complete system. Thus, they are too costly to be applied frequently, up to after each code change. They do not keep also manual changes to the model when recalibrating. In this work, we present the Continuous Integration of Performance Models (CIPM), which incrementally extracts and calibrates the performance model, including parametric dependencies. CIPM responds to source code changes by updating the PM and adaptively instrumenting the changed parts. To allow AbPP, CIPM estimates the parametrized PMPs using the measurements (generated by performance tests or executing the system in production) and statistical analysis, e.g., regression analysis and decision trees. Additionally, our approach responds to production changes (e.g., load or deployment changes) and calibrates the usage and deployment parts of PMs accordingly. For the evaluation, we used two case studies. Evaluation results show that we were able to calibrate the PM incrementally and accurately.

==> externals/cocome_distr_bars.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
interval & analysis \\
50--75 & 0.17 \\
75--100 & 0.13 \\
100--125 & 0.21 \\
125--150 & 0.15 \\
150--175 & 0.13 \\
175--200 & 0.04 \\
200--225 & 0.07 \\
225--250 & 0.05 \\
250--275 & 0.01 \\
275--300 & 0.02 \\
300--325 & 0.01 \\
}\bardataanalysis

\pgfplotstableread[row sep=\\,col sep=&]{
interval & monitoring \\
0--25 & 0.0358601906491 \\
25--50 & 0.0748978665456 \\
50--75 & 0.0694507489787 \\
75--100 & 0.0653654108034 \\
100--125 & 0.200635497049 \\
125--150 & 0.183840217885 \\
150--175 & 0.0903313663187 \\
175--200 & 0.0531093962778 \\
200--225 & 0.0422151611439 \\
225--250 & 0.0267816613709 \\
250--275 & 0.0226963231956 \\
275--300 & 0.0245120290513 \\
300--325 & 0.0236041761235 \\
325--350 & 0.0131638674535 \\
350--375 & 0.00817067635043 \\
375--400 & 0.00499319110304 \\
}\bardatamonitoring

\begin{figure}[!h]
\centering

\begin{tikzpicture}
    \begin{axis}[
            ybar,
            xlabel=Response time (in ms),
            ylabel=Number of occurrences (in percent),
            ytick={0.0, 0.05, 0.1, 0.15, 0.2},
            yticklabels={0.0, 0.05, 0.1, 0.15, 0.2},
            xtick=data,
            bar width=0.01cm,
            symbolic x coords={0--25,25--50,50--75,75--100,100--125,125--150,150--175,175--200,200--225,225--250,250--275,275--300,300--325,325--350,350--375,375--400},
            xtick={0--25,50--75,100--125,150--175,200--225,250--275,300--325,350--375},
            xticklabels={0, 50, 100, 150, 200, 250, 300, 350}
        ]
        \addplot table[x=interval,y=analysis]{\bardataanalysis};
        \addplot table[x=interval,y=monitoring]{\bardatamonitoring};
        \legend{Analysis, Monitoring}
    \end{axis}
\end{tikzpicture}

\caption{Comparison of the analysis results and the monitoring data for CoCoME's "bookSale" service}
\label{fig:bars:booksale}
\end{figure}

==> externals/comparisons/box_plot_teastore.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
  \begin{axis}
    [ylabel = KS-Test,
    boxplot/draw direction=y,
    xtick={1,2,3,4},
    xticklabels={Parameterized (20), Non-parameterized (20), Parameterized (40), Non-parameterized (20)},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[mark = *, mark options = {red},
    boxplot prepared={
      lower whisker=2.214844,
      lower quartile=3.608312,
      median=3.895478,
      upper quartile=4.447298,
      upper whisker=4.666284
    }, color = red
    ] coordinates{(0,4.832228)(0,5.513942)(0,6.29165)(0,5.216712)(0,5.677036)(0,4.981995)(0,5.172095)(0,4.056417)};
    \addplot+[mark = *,mark options = {blue},
    boxplot prepared={
      lower whisker=3.508799,
      lower quartile=5.079821,
      median=5.481519,
      average=5.442438,
      upper quartile=5.971588,
      upper whisker=6.250831
    }, color = blue
    ] coordinates{(0,6.508115)(0,6.486354)(0,6.860059)(0,6.620663)(0,7.312391)(0,7.357306)(0,6.421694)
    (0,6.479597)(0,6.690945)(0,6.661593)(0,7.271025)(0,6.396931)(0,7.035161)(0,7.371248)(0,7.033689)
    (0,7.002645)(0,6.590617)(0,7.171933)(0,6.416259)};
    \addplot+[mark = *,mark options = {green},
    boxplot prepared={
      lower whisker=2.437751,
      lower quartile=3.334956,
      median=4.336029,
      upper quartile=5.068459,
      upper whisker=5.265037
    }, color = green
    ] coordinates{(0,5.826492)(0,5.819791)(0,6.21436)(0,4.47166)};
    
    \addplot+[mark = *,mark options = {orange},
    boxplot prepared={
      lower whisker=3.508799,
      lower quartile=5.079821,
      median=5.481519,
      average=5.442438,
      upper quartile=5.971588,
      upper whisker=6.250831
    }, color = orange
    ] coordinates{(0,6.508115)(0,6.486354)(0,6.860059)(0,6.620663)(0,7.312391)(0,7.357306)(0,6.421694)
    (0,6.479597)(0,6.690945)(0,6.661593)(0,7.271025)(0,6.396931)(0,7.035161)(0,7.371248)(0,7.033689)
    (0,7.002645)(0,6.590617)(0,7.171933)(0,6.416259)};
    
    \end{axis}
\end{tikzpicture}
\caption{Comparison of the KS-Tests for the "train" service}
\label{fig:box:kss:train}
\end{figure}

==> externals/comparisons/kstest_teastore_parametric.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={KS-Test},
    xmin=1, xmax=100,
    ymin=0, ymax=0.5,
    xtick={0, 25, 50, 75, 100},
    ytick={0, 0.1, 0.2, 0.3, 0.4, 0.5},
    legend columns=2, 
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=2
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=point,
    ]
    coordinates {
    (1,0.0881758310937)(2,0.133749788141)(3,0.105472627781)(4,0.0989927604658)(5,0.156418730781)(6,0.102533836953)(7,0.10604767439)(8,0.0980424202804)(9,0.0915353139149)(10,0.0903549550858)(11,0.1712700661)(12,0.143011065107)(13,0.103204063691)(14,0.102700297814)(15,0.0992356159031)(16,0.097397762766)(17,0.174917072226)(18,0.0822256119707)(19,0.157196556984)(20,0.0952670637515)(21,0.119900244546)(22,0.218768916007)(23,0.153392169681)(24,0.117802837704)(25,0.143782838188)(26,0.168431151788)(27,0.0963620526847)(28,0.127633108157)(29,0.159454371565)(30,0.200827461805)(31,0.114864046875)(32,0.137826565943)(33,0.121873562383)(34,0.0971798503668)(35,0.130390305319)(36,0.115127357691)(37,0.0879791046222)(38,0.157895692598)(39,0.125118035883)(40,0.123038788407)(41,0.102200915232)(42,0.133235272754)(43,0.147039417932)(44,0.160398658628)(45,0.108747366892)(46,0.191566184838)(47,0.116831102862)(48,0.132878138544)(49,0.126401297789)(50,0.128722670153)(51,0.140777463015)(52,0.154814653398)(53,0.110360523958)(54,0.0960842352485)(55,0.100151933367)(56,0.148679814048)(57,0.161842328273)(58,0.159312123193)(59,0.113399191303)(60,0.122566644875)(61,0.132194135735)(62,0.119107285538)(63,0.0925764509334)(64,0.10434069393)(65,0.0980226954511)(66,0.134116002034)(67,0.142263504516)(68,0.0954456308564)(69,0.152335899857)(70,0.0973614440328)(71,0.141352509624)(72,0.141606740757)(73,0.142478390354)(74,0.114697586015)(75,0.173996997651)(76,0.121096675458)(77,0.229719014067)(78,0.103411644036)(79,0.154814653398)(80,0.116586160141)(81,0.101822595095)(82,0.143395438367)(83,0.116053485388)(84,0.141125517542)(85,0.152405510762)(86,0.120411733372)(87,0.0968348224014)(88,0.101168857897)(89,0.134249170722)(90,0.0997705866686)(91,0.108519748624)(92,0.108350887388)(93,0.0881697779715)(94,0.112775719716)(95,0.122845088497)(96,0.165946345125)(97,0.131585796954)(98,0.1372152006)(99,0.116495363308)(100,0.0997606720719)
    };
    
\addplot[
    color=blue,
    mark=point,
    ]
    coordinates {
    (1,0.105396600567)(2,0.137119924457)(3,0.132012905257)(4,0.174798495886)(5,0.125961598993)(6,0.0931303116147)(7,0.0796742209632)(8,0.17483160214)(9,0.0770727101039)(10,0.149931507429)(11,0.114160283201)(12,0.0815171545483)(13,0.0738015388068)(14,0.173968029138)(15,0.077235165589)(16,0.140015434647)(17,0.121404121139)(18,0.11328892632)(19,0.0892807680201)(20,0.121517154548)(21,0.130406043437)(22,0.156941353028)(23,0.149790683034)(24,0.0860214038401)(25,0.0970223481272)(26,0.121939498179)(27,0.154513186294)(28,0.0992949323261)(29,0.0831743783444)(30,0.118679571923)(31,0.167149925685)(32,0.136507711678)(33,0.134850487882)(34,0.108243626062)(35,0.109675978269)(36,0.0996180696074)(37,0.0981190479215)(38,0.1187299339)(39,0.163441757723)(40,0.0846661331233)(41,0.117593909984)(42,0.146008813346)(43,0.102425243941)(44,0.250406043437)(45,0.0724803273528)(46,0.125961598993)(47,0.0763987252125)(48,0.115947434687)(49,0.114285489455)(50,0.121404121139)(51,0.124241422726)(52,0.102019200504)(53,0.0946184068528)(54,0.148183821215)(55,0.12679118129)(56,0.0975747560592)(57,0.114897702235)(58,0.139261263996)(59,0.125868406853)(60,0.154315054634)(61,0.143739376771)(62,0.1587299339)(63,0.0948504878816)(64,0.103546978281)(65,0.124071201808)(66,0.130406043437)(67,0.110908089393)(68,0.166046978281)(69,0.146008813346)(70,0.130465848285)(71,0.100015738118)(72,0.0744213595193)(73,0.14534623859)(74,0.130406043437)(75,0.200721613965)(76,0.0993547371734)(77,0.154513186294)(78,0.146463644948)(79,0.123174378344)(80,0.123786591124)(81,0.133130311615)(82,0.128231035568)(83,0.136656043437)(84,0.114285489455)(85,0.146463644948)(86,0.125961598993)(87,0.141066112798)(88,0.148183821215)(89,0.150908089393)(90,0.133789457709)(91,0.114334614866)(92,0.0926754800126)(93,0.111502990242)(94,0.146463644948)(95,0.120485127479)(96,0.125868406853)(97,0.108183821215)(98,0.0990826925671)(99,0.154513186294)(100,0.106381559725)
    };
    
\addplot[
    color=orange,
    mark=point,
    ]
    coordinates {
    (1,0.104673427125)(2,0.128652656338)(3,0.18187906778)(4,0.199761197)(5,0.126859947845)(6,0.232597006886)(7,0.208725264611)(8,0.162902202709)(9,0.174594043784)(10,0.104122838735)(11,0.149789803609)(12,0.127257823286)(13,0.165434115662)(14,0.168219217094)(15,0.103309282756)(16,0.138534540062)(17,0.129063671028)(18,0.200997633292)(19,0.109022664519)(20,0.268043922892)(21,0.133442245743)(22,0.198811715206)(23,0.106505854681)(24,0.162362069847)(25,0.189704619887)(26,0.152520022535)(27,0.242653416677)(28,0.112963069489)(29,0.111011356913)(30,0.147122148445)(31,0.162548895536)(32,0.202589819867)(33,0.185392887434)(34,0.15631231784)(35,0.0988139796492)(36,0.115153522137)(37,0.147191659947)(38,0.163639873191)(39,0.197897491947)(40,0.166733778187)(41,0.16897105713)(42,0.211154090123)(43,0.148943206371)(44,0.125946440106)(45,0.11501750378)(46,0.136218489543)(47,0.140720458148)(48,0.138064203182)(49,0.180829251857)(50,0.142154173078)(51,0.104361466345)(52,0.151069438053)(53,0.212852866672)(54,0.1752720071)(55,0.212198701232)(56,0.146518144764)(57,0.146073017334)(58,0.147656337884)(59,0.132443881986)(60,0.130998875083)(61,0.105091223516)(62,0.16703752123)(63,0.18080665308)(64,0.213975494708)(65,0.162058714884)(66,0.151313194399)(67,0.156617835046)(68,0.187901373532)(69,0.183259647623)(70,0.126446285218)(71,0.15022228979)(72,0.177492850569)(73,0.140002922849)(74,0.165507280915)(75,0.178957920174)(76,0.18370340543)(77,0.160531441062)(78,0.164640309644)(79,0.142996880912)(80,0.134307920438)(81,0.0975449823455)(82,0.211547431002)(83,0.168187094135)(84,0.228855356918)(85,0.170002383144)(86,0.163141355692)(87,0.155974309658)(88,0.167117957399)(89,0.212237720924)(90,0.16911486753)(91,0.161244329761)(92,0.176184175925)(93,0.208114485862)(94,0.201894973667)(95,0.137184128445)(96,0.194947324305)(97,0.167756186298)(98,0.141141023674)(99,0.156675359206)(100,0.165005602802)
    };    
    
\addplot[
    color=green,
    mark=point,
    ]
    coordinates {
    (1,0.237717696988)(2,0.318061353626)(3,0.207222569193)(4,0.192341616812)(5,0.26256532188)(6,0.259298716572)(7,0.24330665308)(8,0.261163795937)(9,0.244947844761)(10,0.236786061257)(11,0.298281178095)(12,0.272632049905)(13,0.236058955873)(14,0.250409827683)(15,0.251097067911)(16,0.261494094186)(17,0.232632049905)(18,0.300204210769)(19,0.205965383239)(20,0.282566892381)(21,0.182725622539)(22,0.280503400317)(23,0.200742956486)(24,0.334854272128)(25,0.307170066984)(26,0.309132782197)(27,0.263452727924)(28,0.294854272128)(29,0.324947844761)(30,0.245674950146)(31,0.209233943279)(32,0.300972569193)(33,0.290409827683)(34,0.246953273946)(35,0.210409827683)(36,0.247770938794)(37,0.219847067911)(38,0.222725622539)(39,0.226073044849)(40,0.29383673365)(41,0.218120877435)(42,0.30580665308)(43,0.265938538631)(44,0.265258283479)(45,0.265628081651)(46,0.26256532188)(47,0.311614511428)(48,0.241230505701)(49,0.225449510223)(50,0.222725622539)(51,0.222965178708)(52,0.258561297539)(53,0.252750421844)(54,0.27455665308)(55,0.263743161017)(56,0.228995463809)(57,0.27707649435)(58,0.206674035238)(59,0.271454210769)(60,0.245965383239)(61,0.281520938794)(62,0.240742956486)(63,0.310270938794)(64,0.223452727924)(65,0.254854272128)(66,0.201520938794)(67,0.260245463809)(68,0.308187605461)(69,0.254854272128)(70,0.192632049905)(71,0.296878081651)(72,0.254854272128)(73,0.152632049905)(74,0.289951432068)(75,0.280742956486)(76,0.278651140622)(77,0.211138320952)(78,0.250409827683)(79,0.298101805897)(80,0.259298716572)(81,0.258120877435)(82,0.276058955873)(83,0.245187400931)(84,0.289392289206)(85,0.219899317173)(86,0.253676432991)(87,0.299298716572)(88,0.285965383239)(89,0.280343099657)(90,0.246606585877)(91,0.192632049905)(92,0.259939919211)(93,0.270092367366)(94,0.301342367366)(95,0.287949510223)(96,0.230557349782)(97,0.31707649435)(98,0.236058955873)(99,0.263743161017)(100,0.290409827683)
    };    
    
%\legend{Parameterized (20 Users), Non-Parameterized (20 Users), Parameterized (40 Users), Non-Parameterized (40 Users)}

\legend{P (20 Users), NP (20 Users), P (40 Users), NP (40 Users)}

\end{axis}
\end{tikzpicture}
\caption{Comparison of the KS-Tests for the "train" service}
\label{fig:comp:kss:train}
\end{figure}

==> externals/comparisons/wasserstein_teastore_parametric.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={WS-Distance},
    xmin=1, xmax=100,
    ymin=0, ymax=100,
    xtick={0, 25, 50, 75, 100},
    ytick={0, 20, 40, 60, 80, 100},
    legend columns=1, 
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=point,
    ]
    coordinates {
    (1,11.4761597782)(2,17.1864331372)(3,16.3622733106)(4,21.3752814702)(5,22.2351728772)(6,13.9468929324)(7,19.2004491417)(8,15.9770193216)(9,12.6300664633)(10,19.0606976829)(11,20.7657320646)(12,22.3886074187)(13,16.6082185536)(14,26.147093896)(15,13.3164501319)(16,19.6056057965)(17,38.7047165928)(18,23.2561560253)(19,23.600602891)(20,22.1096583618)(21,22.0906485315)(22,14.9401769933)(23,16.9117212658)(24,15.050573836)(25,21.2579114307)(26,19.5240097092)(27,12.1955569666)(28,17.6341735067)(29,24.4929874579)(30,29.255054357)(31,15.7042777415)(32,14.747200431)(33,26.7931769207)(34,12.8132339411)(35,27.3452004794)(36,19.5581583981)(37,20.8486931309)(38,16.4945975884)(39,25.4381532676)(40,19.6783612988)(41,18.6652169439)(42,23.6265011743)(43,14.4261730951)(44,8.5752524152)(45,19.6020616934)(46,18.7476937604)(47,9.63149197356)(48,27.5222694366)(49,16.2128308031)(50,22.8214964529)(51,15.0624833539)(52,21.2959220116)(53,24.6067589162)(54,15.5483341808)(55,12.8507300065)(56,26.9684541537)(57,11.8014666715)(58,21.4725036924)(59,19.9301167042)(60,10.7575875887)(61,21.0361462192)(62,20.8325615603)(63,12.8457301276)(64,19.1016107358)(65,24.6772491941)(66,15.0907181424)(67,28.5389094695)(68,17.6162441587)(69,21.5400414034)(70,20.2867333721)(71,21.9357249219)(72,22.9260732186)(73,7.74519684753)(74,20.4383519769)(75,22.4123053921)(76,21.790107779)(77,13.2395856033)(78,11.5306608381)(79,18.240911237)(80,17.7961459771)(81,20.285368393)(82,22.6505956272)(83,20.5447719184)(84,11.2035150481)(85,16.3687531779)(86,18.792078279)(87,25.1097098133)(88,24.349168301)(89,20.9223021234)(90,26.8905171788)(91,12.4601771352)(92,14.5047547275)(93,19.7193439626)(94,17.0464244207)(95,22.3562716399)(96,15.5109137793)(97,18.4219903876)(98,15.4320415971)(99,20.1538491804)(100,26.4449220149)
    };
    
\addplot[
    color=blue,
    mark=point,
    ]
    coordinates {
    (1,11.7211237016)(2,13.3997167139)(3,19.6135096003)(4,10.7261525361)(5,27.6297733711)(6,14.533578848)(7,27.7996467355)(8,16.9120428077)(9,20.6799276047)(10,9.02589167376)(11,9.55769996231)(12,9.99842933585)(13,18.1826782606)(14,15.4124974707)(15,20.0331971951)(16,21.968533645)(17,13.9508254081)(18,23.8221167343)(19,17.047349701)(20,12.3204658483)(21,14.9526156752)(22,13.5137638271)(23,14.4468319169)(24,11.5511000944)(25,47.1203808624)(26,16.3295730473)(27,12.6633743086)(28,18.6015926975)(29,18.3100094429)(30,14.108470255)(31,10.4738505528)(32,19.5774441297)(33,18.1872033365)(34,15.4621372364)(35,8.31793573767)(36,15.4208569405)(37,13.6618711281)(38,15.5467831287)(39,9.26375118036)(40,12.8995996308)(41,15.660877086)(42,9.49950897073)(43,23.612625118)(44,32.8779540447)(45,14.480166824)(46,13.8925007869)(47,34.0630395926)(48,9.67785961599)(49,16.2652754171)(50,15.6748027115)(51,14.8136323576)(52,10.4490368272)(53,35.0549077634)(54,9.36571608436)(55,10.8969255622)(56,18.1767485049)(57,11.4700881335)(58,10.7233660461)(59,16.8395133549)(60,12.9550620531)(61,9.38974346868)(62,20.8997450425)(63,35.7554831602)(64,15.6477387697)(65,11.2811646777)(66,10.8841989298)(67,14.3127824992)(68,7.50786203292)(69,15.4882530689)(70,12.8034592383)(71,40.6581586402)(72,14.3256858785)(73,17.6215832546)(74,17.5433805477)(75,13.4643404027)(76,10.7482562166)(77,14.7706014771)(78,8.3344916588)(79,7.5253604029)(80,14.2851872836)(81,10.3704910293)(82,11.1503273528)(83,15.1672526305)(84,15.0885269122)(85,12.9495624803)(86,19.7756468366)(87,18.6955944562)(88,21.6379697828)(89,22.3682294618)(90,12.8022350938)(91,7.05833080399)(92,6.41622757318)(93,23.7510387158)(94,20.8233931382)(95,13.6602210643)(96,15.7138641576)(97,10.6017437834)(98,10.1722818022)(99,12.0888936665)(100,41.9648253069)
    };
    
\addplot[
    color=orange,
    mark=point,
    ]
    coordinates {
    (1,25.3090544493)(2,32.9394357519)(3,30.6337210736)(4,37.1035970798)(5,31.6835019308)(6,43.1217326215)(7,29.2349227915)(8,36.1797371561)(9,43.8389700434)(10,45.981468182)(11,33.6213341462)(12,23.4718563046)(13,32.939020183)(14,54.0275334941)(15,25.8850122754)(16,41.5485537148)(17,33.188985356)(18,48.0545309885)(19,28.5184878542)(20,42.4196180049)(21,48.1444170885)(22,29.2220906753)(23,39.2104347514)(24,43.8852790629)(25,34.8347955745)(26,48.0676106021)(27,38.0249933013)(28,32.0934973046)(29,34.5771528218)(30,54.7241841919)(31,47.6656869252)(32,48.6958832225)(33,37.9761175451)(34,25.4555578152)(35,41.5316927443)(36,40.3276493244)(37,42.5132714208)(38,43.6435780947)(39,27.7717099259)(40,51.1439621236)(41,44.3057627773)(42,48.1157924996)(43,38.0616811218)(44,39.1864881407)(45,49.4110810737)(46,46.8049378739)(47,46.9334263946)(48,33.7168899226)(49,35.4579303109)(50,30.4688665976)(51,22.4151286478)(52,45.3882924273)(53,49.2434095434)(54,26.7430693765)(55,42.5445964829)(56,45.7683540488)(57,41.3877274824)(58,51.865684154)(59,51.9678558451)(60,50.2271866851)(61,38.9688742702)(62,54.3026622013)(63,41.8674604596)(64,34.9787429083)(65,27.626685627)(66,36.9684479532)(67,53.1160488149)(68,29.4636512133)(69,28.9049741593)(70,38.358002144)(71,33.0515227865)(72,50.7465999112)(73,28.5519764472)(74,45.948279871)(75,48.6437948588)(76,51.7150052398)(77,50.0416537696)(78,39.5437577937)(79,33.5807278611)(80,43.7003973467)(81,28.9292143283)(82,38.6164030146)(83,54.9709553714)(84,46.7334464139)(85,34.0723943112)(86,53.9110801591)(87,46.4014378181)(88,27.9972092254)(89,36.2220508244)(90,44.7125140662)(91,44.6895282249)(92,35.260881427)(93,34.47384755)(94,26.1906736444)(95,33.9798598967)(96,36.0366998474)(97,49.1969354264)(98,49.0281277803)(99,30.3322078157)(100,30.3247136646)
    };    
    
\addplot[
    color=green,
    mark=point,
    ]
    coordinates {
   (1,56.6857646878)(2,71.4571732628)(3,46.2849459273)(4,35.4814278775)(5,58.6944976223)(6,57.2981006801)(7,49.4283433864)(8,41.0862451515)(9,55.0388983484)(10,52.9693429463)(11,54.4956897786)(12,56.6825640436)(13,42.5099856829)(14,48.42394718)(15,31.7028445697)(16,56.2266349645)(17,40.468220586)(18,51.4903297778)(19,31.3374794191)(20,46.458759286)(21,45.1711637777)(22,58.9283264304)(23,29.4039538273)(24,46.7443199366)(25,64.031350156)(26,66.5468411018)(27,47.7560119139)(28,67.2713588485)(29,66.5353538375)(30,36.3585644526)(31,37.7645732172)(32,67.5082362271)(33,61.8623546556)(34,41.103537325)(35,37.5917382523)(36,44.1987480277)(37,39.6385181776)(38,56.8739960117)(39,30.6830475526)(40,63.9841179629)(41,43.8744958327)(42,60.216687348)(43,36.8310456614)(44,44.0836524555)(45,51.2727713497)(46,49.8033721941)(47,79.2013795572)(48,59.8207048627)(49,54.0471677569)(50,42.7601216956)(51,44.8144375415)(52,54.638276215)(53,59.0770800736)(54,50.1948261127)(55,34.0768387278)(56,45.8184064986)(57,62.2562616966)(58,46.049571445)(59,61.6951045661)(60,59.0917712328)(61,51.7395722759)(62,46.4218083039)(63,69.9359468477)(64,51.0873025004)(65,54.3819028992)(66,44.2713043923)(67,67.3475260502)(68,62.1293846193)(69,56.0840952089)(70,30.0864575344)(71,62.1851579449)(72,58.4361185253)(73,40.4310643248)(74,71.3627225901)(75,42.2522961088)(76,69.3542440504)(77,24.2525536618)(78,52.1571690443)(79,58.0090679229)(80,46.9223682058)(81,53.4165805083)(82,55.4886391062)(83,50.9076149205)(84,62.1324129468)(85,20.8585242514)(86,33.4808666973)(87,67.8850368155)(88,54.5639668661)(89,55.5467911745)(90,60.6727120724)(91,39.5266612977)(92,49.9140563481)(93,46.203664289)(94,61.8925202156)(95,60.8622666163)(96,36.6332151208)(97,67.3921641867)(98,41.304701897)(99,65.7374290535)(100,58.2486904945)
    };    
    
\legend{Parameterized (20 Users), Non-Parameterized (20 Users), Parameterized (40 Users), Non-Parameterized (40 Users)}

\end{axis}
\end{tikzpicture}
\caption{Comparison of the Wasserstein distances for the "train" service (100 simulation repetitions)}
\label{fig:comp:ws:train}
\end{figure}

==> externals/evolution/evolution_kstest.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={KS-Test},
    xmin=1, xmax=20,
    ymin=0, ymax=1,
    xtick={0, 10, 20},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    mark=point
    ]
    coordinates {
    (1,0.2928476259689923)(2,0.4027879901960784)(3,0.33044149709302323)(4,0.28387661637931033)(5,0.3408988864942529)(6,0.24093083817829458)(7,0.27545118701550386)(8,0.32460039511494254)(9,0.3416757509689923)(10,0.3279281734496124)(11,0.2318157327586207)(12,0.28387661637931033)(13,0.382328003875969)(14,0.2235766882183908)(15,0.3939559108527132)(16,0.36847444282945735)(17,0.3408988864942529)(18,0.2460483284883721)(19,0.344378591954023)(20,0.283203125)
    };

\end{axis}
\end{tikzpicture}
\caption{KS-Tests for the evolution scenario of the TeaStore (10 evolutionary steps)}
\label{fig:evolution:kss}
\end{figure}

==> externals/evolution/evolution_wasserstein.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={WS-Distance},
    xmin=1, xmax=20,
    ymin=0, ymax=100,
    xtick={0, 10, 20},
    ytick={0, 20, 40, 60, 80, 100},
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=5
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    mark=point
    ]
    coordinates {
    (1,42.33577095445688)(2,46.617294730392224)(3,36.77414910368207)(4,36.70267600574701)(5,21.160380747126325)(6,65.49306564922526)(7,69.37026102228653)(8,17.27128232758611)(9,33.08321220930238)(10,34.97883357558098)(11,22.870599856322055)(12,13.265063757183928)(13,26.549282340116346)(14,30.50345725574734)(15,40.67771923449589)(16,12.50290697674419)(17,35.60897090517252)(18,28.625514777131603)(19,23.015512751436674)(20,9.423626077586215)
    };
\legend{#1}

\end{axis}
\end{tikzpicture}
\caption{Wasserstein distances for the evolution scenario of the TeaStore (10 evolutionary steps)}
\label{fig:evolution:ws}
\end{figure}

==> externals/kstest_cocome_all.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={KS-Test},
    xmin=1, xmax=100,
    ymin=0, ymax=1,
    xtick={0, 25, 50, 75, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=point,
    ]
    coordinates {
    (1,0.140249659555)(2,0.17741715842)(3,0.163113935542)(4,0.153812982297)(5,0.134362233318)(6,0.152437585111)(7,0.147526100772)(8,0.153363595098)(9,0.136631865638)(10,0.137539718566)(11,0.164307762143)(12,0.149754879709)(13,0.145710394916)(14,0.13799364503)(15,0.141556967771)(16,0.145683159328)(17,0.147526100772)(18,0.143413527009)(19,0.161062187926)(20,0.163867453473)(21,0.163812982297)(22,0.132078983205)(23,0.139355424421)(24,0.128007262823)(25,0.152492056287)(26,0.152065365411)(27,0.164984112574)(28,0.162932364957)(29,0.136591012256)(30,0.141516114389)(31,0.142986836133)(32,0.157512482978)(33,0.160662732637)(34,0.140263277349)(35,0.15950068089)(36,0.139355424421)(37,0.133908306854)(38,0.149314571039)(39,0.160236041761)(40,0.126645483432)(41,0.156109850204)(42,0.156445755788)(43,0.153840217885)(44,0.124802541988)(45,0.17565592374)(46,0.143840217885)(47,0.145256468452)(48,0.129822968679)(49,0.144707217431)(50,0.176509305493)(51,0.135147526101)(52,0.137072174308)(53,0.13345438039)(54,0.158393100318)(55,0.143881071266)(56,0.136109850204)(57,0.153867453473)(58,0.129822968679)(59,0.155683159328)(60,0.153413527009)(61,0.132078983205)(62,0.130689968225)(63,0.140263277349)(64,0.167004085338)(65,0.157004085338)(66,0.147526100772)(67,0.132051747617)(68,0.139355424421)(69,0.141570585565)(70,0.137539718566)(71,0.156109850204)(72,0.135710394916)(73,0.140703586019)(74,0.172478438493)(75,0.133000453926)(76,0.13748524739)(77,0.176881525193)(78,0.145256468452)(79,0.174693599637)(80,0.13345438039)(81,0.144280526555)(82,0.152423967317)(83,0.140676350431)(84,0.143840217885)(85,0.135256468452)(86,0.140263277349)(87,0.14704493872)(88,0.136137085792)(89,0.12755333636)(90,0.1523876532)(91,0.162877893781)(92,0.141116659101)(93,0.153277349069)(94,0.139328188833)(95,0.163413527009)(96,0.128447571493)(97,0.132532909669)(98,0.147444394008)(99,0.132986836133)(100,0.134362233318)
    };

\end{axis}
\end{tikzpicture}
\caption{KS-Tests for the "bookSale" service}
\label{fig:kss:booksale}
\end{figure}

==> externals/kstest_cocome_single.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Service response time in milliseconds},
    ylabel={CDF},
    xmin=0, xmax=1200,
    ymin=0, ymax=1,
    xtick={0, 200, 400, 600, 800, 1000, 1200},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=blue,
    mark=point,
    ]
    coordinates {
    (16,0.000453926463913)(17,0.00136177939174)(18,0.00544711756695)(19,0.015433499773)(20,0.02088061734)(21,0.0254198819791)(22,0.0267816613709)(23,0.0308669995461)(24,0.0335905583296)(25,0.0376758965048)(26,0.0390376758965)(27,0.0403994552882)(29,0.0408533817522)(30,0.0435769405356)(31,0.0463004993191)(32,0.0540172492056)(33,0.0590104403087)(34,0.0612800726282)(35,0.0644575578756)(36,0.0694507489787)(37,0.0708125283704)(38,0.07308216069)(39,0.0758057194734)(40,0.0767135724013)(41,0.0789832047208)(42,0.0803449841126)(43,0.0853381752156)(44,0.0898774398547)(45,0.0957784838856)(46,0.0998638220608)(47,0.1044030867)(48,0.107126645483)(49,0.108942351339)(50,0.111211983659)(51,0.11257376305)(52,0.115751248298)(53,0.118020880617)(54,0.118928733545)(55,0.120290512937)(56,0.123921924648)(57,0.12755333636)(58,0.133000453926)(59,0.136177939174)(60,0.141171130277)(61,0.144348615524)(62,0.14616432138)(63,0.147526100772)(64,0.148887880163)(65,0.150703586019)(66,0.153881071266)(67,0.155242850658)(68,0.157058556514)(69,0.159782115297)(70,0.163867453473)(71,0.166591012256)(72,0.171584203359)(73,0.176123467998)(74,0.178847026782)(75,0.182932364957)(76,0.186109850204)(77,0.187017703132)(78,0.190195188379)(79,0.191556967771)(80,0.195188379483)(81,0.199273717658)(82,0.201997276441)(83,0.203359055833)(84,0.20653654108)(85,0.209260099864)(86,0.212437585111)(87,0.216068996823)(88,0.219700408534)(89,0.220608261462)(90,0.224693599637)(91,0.226509305493)(92,0.231048570132)(93,0.232864275987)(94,0.236495687699)(95,0.238311393554)(96,0.24012709941)(97,0.244212437585)(98,0.245120290513)(99,0.245574216977)(101,0.250113481616)(102,0.251021334544)(103,0.251929187472)(104,0.255106672719)(105,0.256922378575)(106,0.261461643214)(107,0.267362687245)(108,0.272809804812)(109,0.284611892873)(110,0.293236495688)(111,0.30276895143)(112,0.311393554244)(113,0.32364956877)(114,0.337721289151)(115,0.351339083069)(116,0.360871538811)(117,0.371765773945)(118,0.380844303223)(119,0.388561053109)(120,0.398093508852)(121,0.406718111666)(122,0.4176123468)(123,0.42805265547)(124,0.440308669995)(125,0.44893327281)(126,0.458011802088)(127,0.466636404902)(128,0.476622787108)(129,0.486609169315)(130,0.497049477985)(131,0.507035860191)(132,0.514752610077)(133,0.525192918747)(134,0.530640036314)(135,0.536541080345)(136,0.545619609623)(137,0.552428506582)(138,0.559237403541)(139,0.567408079891)(140,0.576032682705)(141,0.582841579664)(142,0.589196550159)(143,0.59509759419)(144,0.602360417612)(145,0.608261461643)(146,0.611892873355)(147,0.614616432138)(148,0.620971402633)(149,0.627326373128)(150,0.633227417158)(151,0.637766681798)(152,0.641852019973)(153,0.645483431684)(154,0.650022696323)(155,0.653654108034)(156,0.660916931457)(157,0.664094416704)(158,0.66591012256)(159,0.670903313663)(160,0.672719019519)(161,0.677258284158)(162,0.681343622333)(163,0.684975034044)(164,0.687244666364)(165,0.691330004539)(166,0.694961416251)(167,0.698138901498)(168,0.702224239673)(169,0.705855651384)(170,0.709487063096)(171,0.712210621879)(172,0.714934180663)(173,0.717657739446)(174,0.72038129823)(175,0.721743077621)(176,0.726282342261)(177,0.729459827508)(178,0.7308216069)(179,0.732637312755)(180,0.733999092147)(181,0.735814798003)(182,0.738084430322)(183,0.740354062642)(184,0.743077621425)(185,0.746255106673)(186,0.748070812528)(187,0.750340444848)(188,0.75170222424)(189,0.752610077167)(190,0.753971856559)(191,0.756695415343)(192,0.757603268271)(193,0.760780753518)(194,0.762596459374)(195,0.764866091693)(196,0.768497503404)(197,0.769405356332)(198,0.771221062188)(199,0.77258284158)(200,0.774398547435)(201,0.776214253291)(202,0.776668179755)(203,0.777122106219)(204,0.778483885611)(205,0.779845665002)(206,0.78302315025)(207,0.785746709033)(208,0.787562414889)(209,0.788924194281)(210,0.791647753064)(211,0.794371311847)(212,0.795279164775)(213,0.798002723559)(214,0.80163413527)(215,0.802541988198)(216,0.802995914662)(217,0.805719473445)(218,0.807535179301)(219,0.808443032229)(220,0.810258738084)(221,0.811620517476)(222,0.812982296868)(223,0.813890149796)(224,0.814798002724)(225,0.816159782115)(227,0.817521561507)(228,0.818883340899)(229,0.819337267363)(230,0.820245120291)(231,0.823422605538)(232,0.82478438493)(233,0.826600090785)(234,0.827507943713)(235,0.828869723105)(236,0.829777576033)(237,0.832501134816)(240,0.833408987744)(241,0.833862914208)(242,0.834316840672)(243,0.834770767136)(244,0.836586472991)(245,0.837948252383)(246,0.838856105311)(247,0.839763958239)(248,0.840217884703)(249,0.841125737631)(250,0.842487517022)(251,0.84339536995)(252,0.844303222878)(253,0.844757149342)(254,0.846118928734)(255,0.847026781661)(257,0.849296413981)(258,0.849750340445)(260,0.8515660463)(261,0.852473899228)(262,0.854289605084)(263,0.855651384476)(264,0.856559237404)(265,0.857467090331)(266,0.858828869723)(267,0.859282796187)(269,0.860190649115)(270,0.860644575579)(271,0.861098502043)(272,0.86200635497)(273,0.863822060826)(274,0.864729913754)(275,0.866091693146)(276,0.867453472537)(277,0.868361325465)(278,0.869269178393)(279,0.871538810713)(280,0.873808443032)(281,0.875170222424)(284,0.876532001816)(286,0.878347707671)(288,0.879255560599)(289,0.879709487063)(290,0.881071266455)(291,0.881979119383)(292,0.88288697231)(293,0.884702678166)(294,0.886518384022)(295,0.886972310486)(296,0.88742623695)(297,0.887880163414)(298,0.888334089877)(299,0.888788016341)(300,0.890149795733)(301,0.891057648661)(302,0.89332728098)(303,0.894689060372)(304,0.896958692692)(305,0.89786654562)(306,0.899228325011)(307,0.900590104403)(308,0.901044030867)(309,0.901951883795)(310,0.902859736723)(312,0.903313663187)(313,0.904675442578)(314,0.905129369042)(317,0.90603722197)(318,0.907399001362)(319,0.90830685429)(320,0.909668633681)(321,0.910576486609)(322,0.911030413073)(323,0.911484339537)(324,0.912846118929)(325,0.913300045393)(326,0.913753971857)(328,0.914661824784)(330,0.915569677712)(331,0.91647753064)(332,0.916931457104)(333,0.918293236496)(335,0.919655015887)(336,0.920562868815)(337,0.922832501135)(338,0.923286427599)(339,0.92464820699)(340,0.925102133454)(341,0.925556059918)(344,0.926009986382)(349,0.926463912846)(352,0.92691783931)(355,0.927825692238)(356,0.928279618702)(361,0.928733545166)(362,0.929641398094)(367,0.931457103949)(368,0.932364956877)(369,0.933272809805)(370,0.933726736269)(371,0.934180662733)(372,0.934634589197)(375,0.935542442124)(377,0.935996368588)(378,0.93735814798)(379,0.937812074444)(380,0.938266000908)(381,0.938719927372)(389,0.939173853836)(395,0.9396277803)(401,0.940081706764)(402,0.940535633227)(403,0.940989559691)(407,0.941897412619)(412,0.942805265547)(415,0.943259192011)(426,0.944167044939)(428,0.944620971403)(430,0.945074897867)(431,0.94552882433)(436,0.945982750794)(437,0.946436677258)(439,0.946890603722)(440,0.947344530186)(443,0.94779845665)(444,0.948252383114)(451,0.948706309578)(456,0.949160236042)(458,0.949614162506)(461,0.95006808897)(463,0.950522015433)(478,0.950975941897)(481,0.951429868361)(484,0.951883794825)(488,0.952337721289)(496,0.952791647753)(497,0.953245574217)(498,0.953699500681)(501,0.954153427145)(504,0.955061280073)(518,0.955515206537)(520,0.955969133)(528,0.956423059464)(534,0.956876985928)(537,0.957330912392)(538,0.957784838856)(542,0.95823876532)(565,0.958692691784)(567,0.959146618248)(569,0.959600544712)(571,0.96050839764)(578,0.960962324103)(592,0.961416250567)(605,0.961870177031)(623,0.962324103495)(633,0.962778029959)(639,0.963231956423)(665,0.963685882887)(672,0.964139809351)(674,0.964593735815)(677,0.965047662279)(684,0.965501588743)(688,0.965955515207)(702,0.96640944167)(704,0.966863368134)(760,0.967317294598)(762,0.967771221062)(767,0.968225147526)(779,0.96867907399)(797,0.969133000454)(801,0.969586926918)(808,0.970040853382)(812,0.970494779846)(817,0.97094870631)(827,0.971402632773)(880,0.971856559237)(882,0.972310485701)(885,0.972764412165)(888,0.973218338629)(896,0.973672265093)(907,0.974126191557)(935,0.974580118021)(960,0.975034044485)(968,0.975487970949)(969,0.975941897413)(970,0.976395823877)(974,0.97684975034)(1002,0.977303676804)(1003,0.977757603268)(1030,0.978211529732)(1062,0.978665456196)(1065,0.97911938266)(1138,0.979573309124)(1170,0.980027235588)(1254,0.980481162052)(1265,0.980935088516)(1277,0.98138901498)(1306,0.981842941443)(1335,0.982296867907)(1340,0.982750794371)(1352,0.983204720835)(1376,0.983658647299)(1440,0.984112573763)(1454,0.984566500227)(1462,0.985020426691)(1535,0.985474353155)(1536,0.985928279619)(1539,0.986382206083)(1736,0.98729005901)(1748,1.0)
    };
\addplot[
    color=red,
    mark=point,
    ]
    coordinates {
    (56,0.01)(58,0.02)(62,0.03)(63,0.04)(65,0.06)(66,0.07)(67,0.1)(68,0.11)(69,0.12)(70,0.14)(71,0.17)(77,0.18)(81,0.19)(82,0.2)(88,0.21)(90,0.23)(93,0.24)(95,0.25)(97,0.27)(98,0.29)(99,0.3)(101,0.33)(103,0.34)(105,0.35)(107,0.36)(109,0.37)(113,0.38)(115,0.39)(116,0.4)(117,0.41)(120,0.43)(121,0.45)(122,0.46)(123,0.48)(124,0.5)(125,0.51)(129,0.52)(133,0.54)(134,0.57)(135,0.58)(137,0.6)(138,0.61)(142,0.62)(143,0.63)(144,0.64)(146,0.65)(149,0.66)(151,0.67)(152,0.7)(154,0.71)(158,0.72)(160,0.74)(163,0.75)(167,0.76)(168,0.78)(170,0.79)(175,0.8)(181,0.81)(191,0.82)(195,0.83)(209,0.84)(212,0.85)(214,0.87)(219,0.88)(220,0.89)(223,0.9)(227,0.91)(228,0.92)(242,0.93)(246,0.94)(247,0.95)(282,0.96)(287,0.97)(289,0.98)(338,0.99)(496,1.0)
    };
    
\legend{Monitoring,Simulation of calibrated AM}

\end{axis}
\end{tikzpicture}
\caption{\ac{CDFs} for the "bookSale" service (one iteration)}
\label{fig:cdo:booksale}
\end{figure}

==> externals/kstest_teastore_all.tex <==
\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={KS-Test},
    xmin=1, xmax=100,
    ymin=0, ymax=1,
    xtick={0, 25, 50, 75, 100},
    ytick={0, 0.2, 0.4, 0.6, 0.8, 1.0},
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=point,
    ]
    coordinates {
    (1,0.205597014925)(2,0.13302238806)(3,0.276026119403)(4,0.258582089552)(5,0.169402985075)(6,0.275093283582)(7,0.238432835821)(8,0.192164179104)(9,0.228638059701)(10,0.240858208955)(11,0.168843283582)(12,0.224067164179)(13,0.270615671642)(14,0.334888059701)(15,0.387593283582)(16,0.269496268657)(17,0.236847014925)(18,0.223320895522)(19,0.211847014925)(20,0.303358208955)(21,0.160447761194)(22,0.161819932595)(23,0.223414179104)(24,0.231436567164)(25,0.162779850746)(26,0.189558257102)(27,0.197854477612)(28,0.174347014925)(29,0.172294776119)(30,0.177985074627)(31,0.290671641791)(32,0.299347014925)(33,0.21072761194)(34,0.338992537313)(35,0.374347014925)(36,0.236287313433)(37,0.282462686567)(38,0.323973880597)(39,0.233675373134)(40,0.245149253731)(41,0.205597014925)(42,0.319589552239)(43,0.262406716418)(44,0.169402985075)(45,0.24197761194)(46,0.209235074627)(47,0.272108208955)(48,0.272108208955)(49,0.209608208955)(50,0.242164179104)(51,0.293843283582)(52,0.30447761194)(53,0.21072761194)(54,0.205597014925)(55,0.129850746269)(56,0.200186567164)(57,0.189085820896)(58,0.272108208955)(59,0.267537313433)(60,0.269682835821)(61,0.227425373134)(62,0.238432835821)(63,0.207835820896)(64,0.154291044776)(65,0.216884328358)(66,0.227891791045)(67,0.29085219066)(68,0.267910447761)(69,0.288246268657)(70,0.211007462687)(71,0.279384328358)(72,0.210354477612)(73,0.245733028406)(74,0.190858208955)(75,0.209608208955)(76,0.173973880597)(77,0.292537313433)(78,0.302145522388)(79,0.144682835821)(80,0.174347014925)(81,0.226399253731)(82,0.217308618199)(83,0.231343283582)(84,0.203171641791)(85,0.145242537313)(86,0.184794776119)(87,0.170209436688)(88,0.282655272027)(89,0.263805970149)(90,0.168650698122)(91,0.17947761194)(92,0.219402985075)(93,0.174720149254)(94,0.183115671642)(95,0.237126865672)(96,0.205597014925)(97,0.30447761194)(98,0.245335820896)(99,0.242444029851)(100,0.158115671642)
    };

\end{axis}
\end{tikzpicture}
\caption{KS-Tests for the "train" service (100 simulation repetitions)}
\label{fig:kss:train}
\end{figure}

==> externals/performance_details.tex <==
\pgfplotstableread{
0   0  0  0   0   0
25000   0.376  3.000  0.721   25000   4.097
100000   1.570 6.899  1.158   100000   9.627
200000   3.018  7.229  1.860   200000   12.107
300000   4.463  7.692  1.994   300000   14.149
400000   5.950  7.712   1.808   400000   15.470
500000   6.290  7.899   1.802   500000   15.991
600000   8.410  7.991   1.771  600000   18.172
700000   9.972  8.194   1.942   700000   20.108
800000   12.156  8.077   1.806   800000   22.039
900000   13.253  8.349  1.898   900000   23.500
1000000  14.780  9.160   1.917  1000000   25.857
}\datatable


\begin{figure}[!h]
\centering
\begin{tikzpicture}
\begin{axis}[
    ylabel=Execution time in seconds (s),
    xtick={200000, 400000, 600000, 800000, 1000000},
    enlarge y limits=false,
    enlarge x limits=0.05,
    ymin=0,ymax=40,
    xmin=0, xmax=1000000,
    ytick={10, 20, 30, 40},
    ybar stacked,
    bar width=10pt,
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      }
]
\addplot table[x index=0,y index=1] \datatable;
\addplot table[x index=0,y index=2] \datatable;
\addplot table[x index=0,y index=3] \datatable;
\legend{Loading Records, RD Calibration, UM Extraction}
\end{axis}
\begin{axis}[
    xlabel=Number of monitoring records,
    enlarge y limits=false,
    enlarge x limits=0.05,
    xmin=0, xmax=1000000,
    xtick=\empty,
    ytick=\empty,
    ymin=0,ymax=40,
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
]

\addplot+[forget plot] table[x index=4,y index=5] \datatable;
%\addplot+[forget plot] table[x index=0,y index=4, restrict x to domain=4:5] \datatable;
%\addplot+ table[x index=0,y index=4, restrict x to domain=7:10] \datatable;
\end{axis}
\end{tikzpicture}
\vspace{-0.2 cm}
\caption{Detailed performance information for an increasing number of monitoring records}
\label{fig:perf:details}
\vspace{-0.5 cm}
\end{figure}

==> externals/wasserstein/wasserstein_cocome_all.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}
\begin{axis}[
    xlabel={Repetition number},
    ylabel={WS-Distance},
    xmin=1, xmax=100,
    ymin=0, ymax=100,
    xtick={0, 25, 50, 75, 100},
    ytick={0, 20, 40, 60, 80, 100},
    legend style={
        at={(0.5,-0.2)},
        anchor=north,
        legend columns=-1
      },
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=red,
    mark=point,
    ]
    coordinates {
    (1,22.400235474353163)(2,23.533760780753546)(3,29.805591806627344)(4,17.853977530640048)(5,24.98883624602816)(6,25.95961472991379)(7,31.3685315478893)(8,18.876134816159787)(9,22.927726395823896)(10,24.052201543349984)(11,19.954805946436704)(12,24.572443826600107)(13,17.261192124375867)(14,24.155937925556078)(15,24.049109169314594)(16,28.005915229232645)(17,30.92310201997254)(18,17.051662505674095)(19,18.049293576940553)(20,21.87515603722199)(21,24.855495347253765)(22,16.398079323649583)(23,27.954961983658666)(24,29.27549080798914)(25,24.505858488424895)(26,24.800541874716313)(27,34.44815308670006)(28,35.20399738992307)(29,14.583933840217892)(30,27.419328756241555)(31,19.903483885610548)(32,15.82261404902407)(33,37.52036995006813)(34,25.15569677712213)(35,17.60226112119837)(36,19.612176577394496)(37,25.03381752156152)(38,22.190932818883436)(39,24.187627666817995)(40,30.293591125737652)(41,23.896802655469827)(42,23.6891880390377)(43,31.16948479346354)(44,16.93010950975943)(45,22.040966863368148)(46,20.425314911484357)(47,23.19506071266457)(48,41.23836813436231)(49,20.998326146164345)(50,18.941769745801246)(51,22.92362687244668)(52,22.37119836586475)(53,21.37230481162054)(54,23.13060315478894)(55,22.54618701770314)(56,32.49997162959603)(57,29.432435882887003)(58,19.118176917839335)(59,23.92372616886066)(60,22.03323592827966)(61,16.67161257376307)(62,19.720977076713595)(63,20.92575465274627)(64,25.107467090331415)(65,24.19423797094872)(66,32.7148206990468)(67,20.162307081252866)(68,27.23337494325921)(69,21.696706196096265)(70,21.911257376305052)(71,20.290456196096216)(72,15.419115978211579)(73,23.6750879482524)(74,31.62620574216979)(75,22.257291193826607)(76,27.953231389015052)(77,23.36118361325467)(78,31.250836926917867)(79,16.861481502496616)(80,21.294513163867475)(81,17.381808896958713)(82,22.016554130730828)(83,30.575649682251512)(84,23.516015093054936)(85,18.41856275533366)(86,23.902278143440792)(87,21.342913073082187)(88,25.584033136631884)(89,24.672080685429005)(90,28.68883340898777)(91,20.86794995460737)(92,36.17198138901508)(93,29.734694167044996)(94,17.041122900590118)(95,20.776909328188854)(96,31.736311280072655)(97,17.81177655469816)(98,31.200082274171606)(99,24.097650930549268)(100,21.252723558783494)
    };

\end{axis}
\end{tikzpicture}
\caption{Absolute Wasserstein distance (between the monitoring and the simulation results) for CoCoME's "bookSale" service (100 simulation repetitions)}
\label{fig:ws:booksale}
\end{figure}

==> sections/Evaluation.tex <==
\input{evaluation/cocome_results.tex}
\input{evaluation/teastore_results.tex}
\vspace{-0.4 cm}
\section{Evaluation}
\label{evaluation}
 % and artificial examples \cite{jaegers}. Due to lack of space, this paper presents only the evaluation results of CoCoME and TeaStore. The results of the artificial case study are included in \cite{jaegers}.
%\footnote{see \url{https://blinded-link} for more detail on the implementation and evaluation.}.
This section introduces the evaluation goals, setup, environment and the results of the evaluation:
\vspace{-0.3 cm}
\subsection{Evaluation Goals}
The evaluation considers three aspects of our approach:
\begin{itemize}[leftmargin=*]
    \item Accuracy of the incremental calibration: We calculate the accuracy of the calibrated models by using the monitoring data as reference and also consider an evolution scenario to include multiple calibration iterations. In particular, we analyze whether the parametric dependencies are recognized by the calibration pipeline.
    \item The time the calibration pipeline needs to derive changes and apply them to the model.
    \item Quantification of the overhead introduced by the monitoring. This allows us to make statements on whether the approach can be applied in practice.
\end{itemize} 

% In the evaluation we considered three aspects of our approach:
% \begin{itemize}
%   \item The incremental calibration of the models: We calculated the accuracy of the incremental calibrated models by using the monitoring data as reference. For this purpose, we considered an evolution scenario to include multiple calibration iterations.
% \item The parametric dependencies: we made sure that the parametric dependencies were recognized by the calibration pipeline. We apply cross-validation and use the correlation coefficient metric to validate the linear regression and both precision and recall metric to validate decision trees.
% Alternative: We varied the usage behavior  during the monitoring, so that the accuracy of the resulting model implicitly indicates whether all parametric dependencies have been detected.
% \item The monitoring overhead: We quantified the monitoring overhead and the time needed for calibration. This allows us to make statements on whether the approach can be applied in practice without noticeably affecting the performance.
% \end{itemize}
%\input{externals/seff_booksale.tex}
\vspace{-0.4 cm}
\subsection{Experiment Setup}
\label{evaluation:setup}
The general procedure for evaluating our approach is structured as follows:\\
%\begin{enumerate}[leftmargin=*]
    1. We monitor the application over a defined period of
    time (e.g., 60 minutes) and perform a load test at the same time to artificially simulate user interactions. \\
    2. We run the monitoring in combination with the load test two times. First, we apply a fine-grained monitoring, whose results are passed to the
    calibration pipeline for adjusting the architecture model (training set). Second, we only observe service calls (coarse-grained monitoring). These data is used to estimate the accuracy of the calibrated model (validation set). This procedure prevents the monitoring overhead from falsifying the evaluation results. During the calibration we also recorded the execution times of the different parts in the pipeline and the overhead which is caused by the monitoring. \\
    3. We adjust the usage model according to the validation set and perform a fixed number of simulations of the updated architecture
    model (100 repetitions). A single execution would not be sufficient here, since the simulation samples from stochastic distributions and one result may not be representative. Afterwards we compare the results of the
    simulations with the validation set. Both are distributions,
    therefore we use the \ac{KS-Test} \cite{KSTest}, the Wasserstein metric \cite{majewski_et_al:LIPIcs:2018:9327} and conventional statistical measures, such as the quartiles, to determine the 
    similarity. The lower the \ac{KS-Test}, the higher is the accuracy of the updated architecture model. We are aware that the KS test is not the optimal choice in our specific case, which is why we also used alternative metrics such as the Wasserstein distance to confirm the results. The Wasserstein metric, on the other hand, is rather a distance measure that quantifies the effort needed to transfer one distributions into the other. If we want to compare the accuracy of two simulation distributions (using the monitoring data as reference), this metric is very well suited, but as an absolute number it is difficult to interpret. Therefore, we just used this metric as an additional measure to confirm the results.
    \begin{comment}
    The self-validation executes this step automatically, but only one simulation is triggered. Therefore, we show more reliable results (the results of 100 simulations using an additional validation set) supplementary to the self-validation results.
    \end{comment}
\input{externals/seff_booksale.tex}
\vspace{-0.3 cm}
\subsection{Evaluation Environments}
We evaluated our approach using two case studies: \ac{CoCoME}~\cite{cocome} and
TeaStore \cite{teastore}. %
%This section provides some information about the used case studies.
%\subsubsection{CoCoME}
%\label{sec:Env:Cocome}
 \ac{CoCoME}  is a trading system which is designed for the use in supermarkets. It supports several processes like scanning products at a cash desk or processing sales using a credit card. We used a cloud-based implementation of \ac{CoCoME} where the enterprise server and
the database run in the cloud.
%\subsubsection{TeaStore}
%\label{sec:Env:Teastore}
\begin{comment}
TeaStore is a micro-service based reference application
\cite{teastore}. It implements a web shop where you can buy
different kinds of tea. Besides, the TeaStore supports user
authentication and automatic recommendations. Amongst others, it is designed to
evaluate approaches in the field of performance modelling \cite{teastore}.


% In future work, we will integrate earlier approaches to import existing source code \cite{langh} into the current \vitruv platform. 
\end{comment}

Additionally, we evaluated our approach using the aforementioned running example of  TeaStore case study (cf. \Cref{Running Example}). 
%\subsubsection{Limitation of the used case studies}
Because of the fact that \ac{CoCoME} and TeaStore are not implemented using the \vitruv platform, we instrument the changed parts of the source code manually. In future work, we will integrate earlier approaches \cite{leonhardt2015a} into the current \vitruv platform to import existing source code \cite{leonhardt2015a} into \vitruv VSUM, which allows using the automatic change-based adaptive instrumentation.
%\vspace{-0.2 cm}
\subsection{Model Accuracy Evaluation}
\label{evaluation:accuracy}
%This section represents the evaluation of the accuracy of the calibration based on CoCoMe, TeaStore.
%In this section we evaluated the accuracy of the calibration based on \ac{CoCoME} and the TeaStore.


First, with the help of CoCoME, we validated the basic functionality and performed initial measurements to assess the accuracy of the adapted models. In the second step, we used the TeaStore case study to evaluate the incremental calibration and ensure that parametric dependencies were considered in the generated models.
\subsubsection{CoCoME case study}
% first evaluation Scenario
In the evaluation scenario using \ac{CoCoME}, we suppose that the ``bookSale'' service  is newly added. According to our assumption, we instrument this service and all services
that are subsequently called by it. 
The ``bookSale'' service is responsible for processing a sale after a user submitted his payment. As input, this service receives a list of the purchased products including all information related to the purchase. In the next step, we performed a load test which simulates user purchases. We used the resulting monitoring data to calibrate our initial architecture model.

The service consists of several internal and external actions and two loops. We also monitored and calibrated the behavior  of all external actions to make the resulting model more accurate.
Figure \ref{fig:seff:booksale} visualizes the structure of the calibrated "bookSale" service
of \ac{CoCoME}. For reasons of simplification, we focused on the structure and omitted certain details.
%end of first evaluation Scenario
As described in the experiment setup, we performed 100 simulations and
compared the distribution of the monitoring with the results of the simulations.
Table \ref{table:cdf} shows the quartiles
for both the monitoring and the simulation results for a single example execution.% of the self-validation process).
\input{externals/cdf_cocome_table.tex}
In addition, a KS test value of \textbf{0.1321} and a Wasserstein distance of \textbf{13.7726} were obtained by comparing the two distributions. It is well visible that the two distributions are very close to each for the first, second and third quartile. The discrepancy in the minimum and maximum values of the distributions arises because we limited the time spent for simulation.
%Increasing the simulation time also increases the probability that outliers will be observed. %Because we also paid attention to the performance in the self-validation, the time for the simulation necessarily had to be limited.
%As mentioned earlier, we performed 100 simulations to increase the reliability of the outcome. That is why we performed another 100 repetitions and calculated the KS test for each of them. We only used the KS test here because we just want to get a general idea about the accuracy of the derived models. 
The average of the KS tests over all 100 simulation runs 
is approximately \textbf{\cocomeavg}, the minimum \textbf{\cocomemin} and the maximum
\textbf{\cocomemax}. From these values it follows that our approach provided a model which represents the monitored behavior  in our scenario well.

\subsubsection{TeaStore case study}
%running example changes
%\input{externals/seff_train.tex}
%second  evaluation Scenario
For the TeaStore case study, we examined the "Recommender" part (cf. \Cref{Running Example}).
\begin{comment}
The Recommender is divided into a service that calculates the
recommendations for a certain shopping cart (recommend service) and a service
that derives information from the previous orders (train service).
\end{comment}
We monitored the "train" service and calibrated it. Furthermore, we modified the application so that the "train" service is executed when a user placed an order. This causes the number of users to have a direct impact on the service response times, as the number of orders in the database grows faster and therefore a higher number of orders have to be processed within the service.

\begin{comment}
Normally the "train" service only receives the past orders and the associated ordered items as input. We
extended it and added a parameter (enum) indicating which Recommender
implementation is used. This allows us to specify a single \ac{SEFF} that is valid for all Recommender implementations.
\end{comment}
Figure \ref{fig:seff:train} shows the simplified layout of the \ac{SEFF}. Except for the last Internal Action, the behavior  is exactly the same for all Recommender types.
%The \ac{SEFF} contains a loop followed by two Internal Actions and one External Action.
% end of 2nd
% 3 incremental calibration

We also considered an evolution scenario for the TeaStore to evaluate the incremental calibration. This means that the calibration of the models is executed several times. In our considered evolution step, new Recommender implementations are added or existing ones were removed.

% the goal of 4, Accuracy of parametrized PM 
In the following, we compared the accuracies of a parameterized and a non-parameterized model. 
% mit 3 integrieren
In the second step, we analyzed the behavior and accuracy of the incrementally calibrated models when executing evolutionary scenarios (e.g., Recommender implementations are added or removed).

%setup o PPM nd NPPM
In order to confirm the recognition of parametric dependencies, we first monitor the service as previously described in section \ref{evaluation:setup} fine granular (F1) and subsequently coarse granular (C1). We \textbf{only} use the resulting fine granular monitoring data (F1) to calibrate two models: one with parametric dependencies using our incremental calibration and one without parametric dependencies using the distributions of the observed values. 
%results PPM
The results confirmed that our calibration was able to detect the parametric dependencies, e.g. the RD of the internal action \textit{trainForRecommender} (the \nth{4} action in train SEFF) is related to the type of recommendation implementation as well as to the number of ordered elements.
%results accuracy PPM, 4/What if scnario 
To compare the accuracy of the parameterized model with the non-parameterized model, we predict the performance for a what-if scenario, i.e. what the performance would be if the load is changed from 20 concurrent users to 40 concurrent users. To have a baseline, we measure the performance by applying the load of 40 users (performing coarse granular monitoring (C2)). Then we compare the simulation results with the monitoring data, i.e. (C1) as reference for the first load (20 users) and (C2) for the second load. 
%The additional load increases the response times of the Recommender service, as the database populates faster and more orders have to be processed by the Recommender implementations.
Table \ref{table:train:kss} shows the comparison of the KS tests and the Wasserstein distances between the parameterized and the non-parameterized model. It can be seen that both models are very accurate for the standard load of 20 users. However, it can be stated that the non-parametric model loses significantly more accuracy than the parameterized model, when the load changes to 40 users.
%\input{externals/comparisons/kstest_teastore_parametric.tex}
%\input{externals/comparisons/box_plot_teastore.tex}
\input{externals/comparisons/teastore_kstest_table.tex}
\begin{comment}
We confirmed this first impression by using Wasserstein distance as an alternative metric. We included the results in the Appendix in Figure \ref{fig:comp:ws:train} and we also summarized the results there in tabular form (see table \ref{table:teastore:param:20} and table \ref{table:teastore:param:40}).
\end{comment}
%Again, the same conclusions can be drawn here: the parameterized model provides more accurate results for varying load scenarios, since it produces lower Wasserstein distances for the scenario with 40 users. The results are summarized in an aggregated and tabular form in the appendix (see Table \ref{table:teastore:param:20} and Table \ref{table:teastore:param:40}). %

%set up of 3 scenario results
In order to evaluate the incremental calibration, we simulated an evolution scenario for the TeaStore application. At the beginning of the scenario, the TeaStore contains a single implementation of the "train" service. Then we perform 15 minutes of fine-granular monitoring and use the resulting data to calibrate the model. After that we monitor the service for another 15 minutes coarse granular. The coarse granular monitoring data is used as reference for the estimation of the accuracy of the calibrated model. In the next step, we add another implementation of the "train" service and again, just like before, we perform a fine granular and a coarse granular monitoring for 15 minutes each. If all implementations of the "train" service have already been added, one of them will be randomly removed again. We repeat this procedure over several iterations and calculate the accuracy of the calibrated model for each iteration. In addition, the database fills up more and more over time, which leads to increasing response times. This adds an extra level of difficulty to the calibration process.

\input{externals/evolution/evolution_table.tex}
We performed 10 consecutive iterations and calculated the accuracy for each of them. As before, we calculated the KS test and confirmed the results using Wasserstein distance.
% results of 3
Table \ref{table:evol} lists the aggregated results. We omitted the values of some iterations because these were always very similar to the previous ones.
The values are slightly higher than before where we did not apply any changes to the application. However, it can be seen that the accuracy of the models is almost constant throughout the evolutionary steps. From this, it can be concluded that the automated calibration can handle changes of the observed services in the TeaStore.

%We also measured the time the calibration pipeline needs to derive changes and apply them to the model. In addition, we analyzed how time-consuming the monitoring is.
\vspace{-0.3 cm}
\subsection{Calibration Performance}
For both \ac{CoCoME} and TeaStore we computed how much time the individual parts of the pipeline took to complete. For the TeaStore, we also distinguished between the two states within the evolution scenario (before and after the first evolution step). The results are shown in table \ref{table:exec}.
\begin{table}[h]
    \centering
    \caption{Execution times of the pipeline parts}
    \begin{tabular}{|c|c|c|c|}
    \hline 
    Measure & CoCoME & TeaStore (1) & TeaStore (2) \\ \hline \hline
    Record Count & \cocomerecords & \teastorerecords & \teastoreitZrecords \\ \hline \hline
    Load Records & \cocomeloading & \teastoreloading & \teastoreitZloading \\ \hline
    RD Calibration & \cocomecalibration & \teastorecalibration & \teastoreitZcalibration \\ \hline
    UM Adjustment & \cocomeusage & \teastoreusage & \teastoreitZusage \\ \hline
    Self-Validation & \cocomeselfvalidation & \teastoreselfvalidation & \teastoreitZselfvalidation \\ \hline \hline
    \textbf{Total} & 17.213s & 10.826s & 2.199s \\ \hline
    \end{tabular}
    \label{table:exec}
\end{table}

We can see that the required time strongly depends on the number of monitoring records and the complexity of the observed service. It has already been shown for iObserve that the derivation of the usage model scales linearly with the number of monitoring records \cite{heinrich2015runtime}. In all considered cases, the execution of the whole pipeline took less than 20 seconds. %, thus the measured times are not problematic. 
It can also be observed that the adaptive monitoring limits the number of monitoring records and accordingly the second iteration of the TeaStore monitoring produces far less records, which results in significantly lower execution times.
To gain detailed insights about the performance of the pipeline, we also examined the behavior for an increasing number of monitoring records. For this purpose, we generated monitoring data with the help of \ac{CoCoME} case study and executed the pipeline several times. The results showed that the execution time of the pipeline scales linearly up with the number of monitoring records, plus an additional constant overhead (see Table \ref{table:perf}).
\input{externals/performance_details_table.tex}
\subsection{Monitoring Overhead}
Kieker only introduces a small overhead, the recording and storing of one record takes on average less than 5 microseconds \cite{kieker}. However, due to the fine-grained instrumentation, a single service call can cause a lot of monitoring records.

We also measured the overhead caused by the monitoring. For CoCoME's "bookSale" service the average monitoring overhead was \cocomeoverhead (fine-grained), \cocomeoverheadsec (coarse-grained) and for TeaStore's Recommender.train service the measured overhead on average amounts to \teastoreoverhead (fine-grained), \teastoreoverheadsec (coarse-grained). We can notice that the coarse-grained monitoring has almost no influence on the execution times. The fine-grained monitoring overhead scales up with the complexity of the service. In our case, the overhead of around 1ms had no drastic impact on the performance, since the execution times of the services are significantly higher.

The evolution scenario described for the TeaStore shows very well that the adaptive monitoring helps to significantly reduce the monitoring overhead. In the first iteration we instrument the statements of all SEFF elements shown in Figure \ref{fig:seff:train} - (1), (2), (3) and (4). For each additional iteration we just instrument the changed internal action (4). In this case we saved \textbf{at least 75\%} of the monitoring overhead. This is reflected in the times required for calibration, which are considerably lower compared to the first iteration (see \autoref{table:exec}).

In general there is a trade off between the monitoring overhead and the accuracy of the model, but our approach tries to balance them by using the incremental calibration in combination with the adaptive monitoring. Consequently, the calibration time and the monitoring overhead can be kept as small as possible.
